SMARTS: Scalable Multi-Agent Reinforcement Learning Training School for Autonomous Driving

Multi-agent interaction is a fundamental aspect of autonomous driving in the real world. Despite more than a decade of research and development, the problem of how to competently interact with diverse road users in diverse scenarios remains largely unsolved. Learning methods have much to offer towards solving this problem. But they require a realistic multi-agent simulator that generates diverse and competent driving interactions. To meet this need, we develop a dedicated simulation platform called SMARTS (Scalable Multi-Agent RL Training School). SMARTS supports the training, accumulation, and use of diverse behavior models of road users. These are in turn used to create increasingly more realistic and diverse interactions that enable deeper and broader research on multi-agent interaction. In this paper, we describe the design goals of SMARTS, explain its basic architecture and its key features, and illustrate its use through concrete multi-agent experiments on interactive scenarios. We open-source the SMARTS platform and the associated benchmark tasks and evaluation metrics to encourage and empower research on multi-agent learning for autonomous driving. Our code is available at https://github.com/huawei-noah/SMARTS.

==> marl4ad.tex <==
% \section{Multi-agent Reinforcement Learning for AD}
%     Multi-agent reinforcement learning (MARL) \cite{littman1994markov} has been studied for a long time. It is framed with the Markov games, which is derived from the Markov Decision Processes (MDPs) \cite{feinberg2012handbook}, enabling us to describe the framework from the MDPs perspective.
    
%     \paragraph*{Markov Games.} An $N$-agent Markov game, sometimes called a stochastic game, can be formalized by the tuple $(\mathcal{S}, \mathcal{A}, \mathcal{P}, \mathcal{R}, \gamma)$, where $\mathcal{S}$ represents the state space, $\mathcal{A}_i \in \mathcal{A}$ denotes the action space of agent $i \in \{1, \dots, N\}$. The state transition function $\mathcal{P}: \mathcal{S} \times \mathcal{A}_1 \times \cdots \times \mathcal{A}_N \rightarrow \Delta(\mathcal{S})$ characterizes the transition probability of states in time, where $\Delta(\mathcal{S})$ is the probability ranges from 0 to 1 over the whole state space. The reward function for agent $i$ is defined as $\mathcal{R}: \mathcal{S} \times \mathcal{A}_1 \times \cdots \times \mathcal{A}_N \rightarrow \mathbb{R}$. For each agent $i$, its goal is to maximize its payoff with its policy $\pi^i: \mathcal{S} \times \mathcal{A}_1 \times \cdots \times \mathcal{A}_N \rightarrow \Delta(\mathcal{A}_i)$. In general, we express the agent learning purpose as a cumulative discounted reward:

%     \begin{equation}
%         G_{i, t=0:T} = \sum_{t=0}^T\gamma^T\mathbb{E}_{\pi^i, \pi^{-i}, \mathcal{P}}\left[ r^i_t \mid s_t\right]
%     \end{equation}

%     In multi-agent autonomous driving, a core issue is making decisions based on understanding the interactions involving other agents. Alternative solutions in MARL include Centralized Training with Decentralized Training (CTDE) \cite{lowe2017multi}, Multi-agent Coordination \cite{chalkiadakis2003coordination} and Opponent learning \cite{carmel1995opponent}. All of these methods integrate extra information of other agents to learn the multi-agent interactions. There are \cite{bhalla2020deep} ...



==> old-fragments.tex <==
% JL: is the following still worth doing? Not too sure.
% TODO by Yaodong: reconstruct Five AI as partial inspiration of SMARTS; be future-oriented, say that SMARTS 0.5 is only a piece of work in progress.
% 1. Computational
% equilibrium computations: fictitious play for computing a sample Nash equilibrium for zero-sum games, replciator dynamics to solve Nash in symmtetrical game. 
% implication in SMARTS: 
% return the pay-off table for equilibrium computation. 
% in two-player case, provide linear programming, RD, alpha-rank, etc https://arxiv.org/pdf/1905.08085.pdf
% beyong nash equilibrium, huamn-machine, machine-machine , ... ,bounded raitonality
% size of agent number

% 2. Descriptive
% investigate formal models of learning that agree with people’s behavior, or how to represent populations.
%
% implication in SMARTS:
% a. support multiagent immitation learning 
% b. support programmable opponent models 
% c. real-world physics

% 3. Normative
% determining which sets of learning rules are in equilibrium with each other
% 
% implication in SMARTS:
% a. support multi-agent learning, QMIX etc librariries 
% b. support both self-play and adhoc-play, FP with Q-learning
% c. algorithmic evaluation

% -------- focus on multiagent necessiry, opponent modelling needed ---- 
% 4. Prescriptive, cooperative
% 
% how agents should learn, how to do distribtued control in a team game. 
%
% implication in SMARTS:
% a. enable communication: http://www.cs.utexas.edu/~pstone/Papers/bib2html-links/JAIR08-dresner.pdf

% 5. Prescriptive, non-cooperative
%
% how to design anoptimal (or at least effective) agent for a given environment, e.g. fix the opponent type
%
% implication in SMARTS:
% a. define what does high mean? non-regret? or absoluate reward? or other driving metric
% b. changeable opponent types


% Machine learning/AI is the process of converting data into knowledge \citep{shalev2014understanding}. The input to a learning algorithm is training data (e.g. some images containing cats), representing experience, and the output is some knowledge (e.g. some rules about how to detect cats), which usually takes the form of a  computer program that can perform some task (e.g. an automatic cat detector). % JL: not needed.
% In the last decade, sensational advantages have been made by a special kind of machine learning technique -- deep learning \citep{lecun2015deep}.  % JL: not needed.
% Deep learning enables  learning representations  from the data, thus allowing  computer programmes to  automatically discover effective features. % JL: not needed.
% One of the key embodiment of deep learning is the different kind of deep neural networks \citep{schmidhuber2015deep} that can find disentangled representations \citep{bengio2009learning} in high-dimensional data. % JL: not needed.
% Uncountably many breakthroughs in real-world AI applications have been achieved through the usage of deep neural networks, among which, the domains of computer vision \citep{krizhevsky2012imagenet} and natural language processing \citep{devlin2018bert} are probably the biggest beneficiaries. % JL: not needed.

%\begin{figure}[t]
%\centering
%\vspace{-10pt}
%\includegraphics[width=\linewidth]{decision_making}
%\caption{Modern AI applications are now transforming from pure pattern recognition (e.g. detecting a cat in an image) to decision makings (e.g. driving through a traffic intersection safely) where interaction among multiple agents inevitably happens. As a result, each agent has to behave strategically. Furthermore, the problem  becomes more challenging because the current decision  will influence the future outcomes.} 
%\label{fig:decision_making}
%\end{figure} % JL: Good to include a picture of a representative interaction scenario. But we do not need the diagrams. Also, we need to be careful about copyright of pictures from elsewhere. We could use some creative commons pictures for example and attribute appropriately. We should combine this figure/example with the next one.

%On top of feature representations, modern AI applications often require computer programmes to make decisions based on the built knowledge (see Fig. \ref{fig:decision_making}).  % JL: not needed.



%%%%%% SMARTS Implementation %%%%%%

%  (3f) lab -- MA trainer; web-based distributed visualization; ULTRA benchmark and other benchmarks ...
    % \platform{} aims to provide a flexible, realistic, and diversified simulator in the rendering, physics simulation, multi-agent interaction, also a training platform for AD researches. In terms of software architecture, \platform{} is mainly composed of a traffic simulator SUMO \cite{krajzewicz2002sumo} and a physics simulator Panda3D \cite{goslin2004panda3d}, rich learning APIs for AD researches, scenario manager and a benchmark for basic driving scenarios. To support the functionality, \platform{} is designed as a server-client system, where the server runs the traffic and physics simulation, the client rich APIs are implemented in Python for autonomous / social agents interacting with the simulation server. Different from the previous work for driving simulator, our \platform{} support a variety control styles from micro control to macro decision making. Scenarios for autonomous driving can be easily created using a scenario manager, with such a tool, we can customize any type of roads, and traffic. The property of scenario include agent mission, traffics, and OpenStreetMap \cite{haklay2008openstreetmap} styled road-map. A training suit has been implemented for (multi-agent) reinforcement learning researches for AD. Specifically, we implemented some tuned adapter for observation and reward definition for reinforcement learning, also a variety of algorithms implemented based on RLlib \cite{liang2018rllib}. Benchmarks are crucial for evaluate the researches for AD with deterministic settings. In \platform{}, we have also implemented a benchmark which integrates scenarios and evaluation programs.

    % \paragraph*{Environment.} The environments in \platform{} are designed for user interacting with simulation and training autonomous agents. Two alternative Gym-based \cite{brockman2016openai} environments have been implemented for scalable autonomous driving researches. In detail, HiWay-env is a environment with typical Gym APIs for small-scale AD research. For large-scale cases, the RLlibHiWayEnv will be a better choice, which is compatible with Ray \cite{moritz2018ray} and RLlib \cite{liang2018rllib}.

    % \paragraph*{Simulators.} In \platform{}, we separated the physics simulation and traffic simulation into two independent simulators, namely, SUMO for traffic and Panda3D for physics, which to some extent optimizes the efficiency and increases the parallelism of the simulation. Specifically, we apply physics simulation for only the autonomous agents not all vehicles in the environment, because the micro behaviors of other vehicles are not crucial, compared to the autonomous agents. Also, to make the autonomous agents have a good sensing of the surroundings, we do simulation of a variety of sensors, including vision, radar, and route planning. In general, there are three popular approaches to make the autonomous vehicle to see the world -- Visual perception, Lidar perception and mixture of them. With the support of various sensors simulation in \platform{}, users can customize the perception systems on their actual requirements.

    % \paragraph*{Controllers.} To support the autonomous driving broadly, we developed five different controllers for \platform{}, they are \textit{ContinuousController}, \textit{LaneFollowingController}, \textit{ActuatorDynamicController}, \textit{TargetPoseController} and \textit{TrajectoryTrackingController}.

    % \begin{itemize}
    %     \item \textit{ContinuousController}: the continuous controller define 3-dimensional control commands: throttle, brake and steering.
    %     \item \textit{LeanFollowingController}: this controller implemented the underlying logic of micro control, that is, the LaneFollowingController only concerns about the decision making.
    %     \item \textit{ActuatorDynamicController}: the logic of this controller is to control the vehicle using throttle, brake and the steering rate degrees per second.
    %     \item \textit{LaneWithContinuousSpeed}: the controller accepts two control singals - target speed and lane switching signal.
    %     \item \textit{TrajectoryTrackingController}: ...
    % \end{itemize}

    % \paragraph*{Scenario Studio.} \platform{} support automated scenario generation. With the support of scenario studio, users can customize the scenario with customized road map, diversity traffic flow, and mission initialization. ...
    

%%%%%% Description Length argument %%%%%%
 We could consider the need here in terms of description length [cite]: if the behavior over time is interesting, the programs driving the generation of the interaction sequences, the programs that run the social agents better be long and hard to compress, whether such programs are based on handwritten rules and code or neural network models. 
